A Novel Dual-Lidar Calibration Algorithm Using Planar Surfaces

Multiple lidars are prevalently used on mobile vehicles for rendering a broad view to enhance the performance of localization and perception systems. However, precise calibration of multiple lidars is challenging since the feature correspondences in scan points cannot always provide enough constraints. To address this problem, the existing methods require fixed calibration targets in scenes or rely exclusively on additional sensors. In this paper, we present a novel method that enables automatic lidar calibration without these restrictions. Three linearly independent planar surfaces appearing in surroundings is utilized to find correspondences. Two components are developed to ensure the extrinsic parameters to be found: a closed-form solver for initialization and an optimizer for refinement by minimizing a nonlinear cost function. Simulation and experimental results demonstrate the high accuracy of our calibration approach with the rotation and translation errors smaller than 0.05rad and 0.1m respectively.

==> contribution.tex <==
\section{New Contribution}
\label{sec.contribution}

\subsection{Overview of the Method}
Inspired by the previous work \cite{taylor2012mutual,taylor2015motion,taylor2016motion,heng2013camodocal,segal2009generalized}, we combine with motion-based and appearance-based approaches to propose an automatic extrinsic calibration method for multi-lidar sensing system in this paper. This method takes the essential ideas used in hand-eye calibration problem to initialize the extrinsic parameters. Then when overlapping of lidars exists, further refinement is done by making use of the appearance information provided by sensors. To our best knowledge, there is no existing work focusing on motion-based multi-lidar calibration. \\

Considering that this sensing system will be mounted on autonomous vehicles, the calibration method should be friendly to non-expert users and successfully used in natural scenes, like roads and streets. To simplify the problem, we assume that several prior knowledge is known:
\begin{enumerate}
	\item The lidars are synchronized.
	\item The lidars are rigidly mounted.
	\item The lidars' intrinsic parameters are known.
	\item The measurements of lidars have a dominant ground plane.
	\item The lidars undergo a series of known and nondegenerate motion. \\
\end{enumerate}

The first assumption means that the relative transformations of lidars at each timestamp $\textbf{T}_{L_i,k}^{L_1,k-1}$ are synchronized. The second assumption ensures that the extrinsic parameters $\underset{1\leq i\leq N}{\bigcup}\{\textbf{T}_{L_i}^{L_1}\}$ are unique. The third assumption ensures that measurements of lidars are undistorted. The fourth assumption is common in outdoor environments and can be used in further appearance-based refinement. And the final assumption guarantees solvable $\textbf{R}$ and $\textbf{t}$ given by enough data.

\subsection{Contribution}
With assumptions made, the contributions of this paper include the following:
\begin{enumerate}
	\item We propose an automatic multi-lidar extrinsic calibration method that doest not require any initial guess. The method can work on sensors with/without overlapping fields of view.
	\item We present the usage of appearance-based approaches to refine the results of motion-based calibration. 
\end{enumerate}

\subsection{Algorithm}
The automatic calibration method is summarized in Algorithm \ref{alg.proposed_method}. Here we use $\textbf{R}, \textbf{t}$ to express transformation instead of $\textbf{T}$. 
Similar to \cite{taylor2016motion, heng2013camodocal}, the algorithm has three steps: motion estimation (line 1-3), initialization (line 5-18), and refinement (line 19). \\

\subsubsection{Motion estimation}
To calculate the relative transformation of consecutive frames of lidars, lightweight lidar odometry and mapping (LOAM) \cite{zhang2014loam} is used. The odometry part of LOAM is a modified ICP which combines point-to-point and point-to-plane metrics. \\

\subsubsection{Initialization}
\label{subsubsec.initialization}
The function of this step is to get an good initial guess, specially, to solve equ. (\ref{equ.rotation_axes}) and (\ref{equ.ls_translation}). Regarding the rotation, a modified version of the Kabsch algorithm developed in \cite{taylor2016motion} is applied. Once the rotation matrix is known, the translation can be calculated using linear least square techniques. Starting with equ. (\ref{equ.ls_translation}), the terms can be rearranged and combined with information from each timestamps to give equ. (\ref{equ.lls}):
\begin{equation}
\begin{split}
\textbf{t}_{y}^{x} = 
\begin{bmatrix}
\textbf{R}_{x,k}^{x,k-1} - \textbf{I} \\
\textbf{R}_{x,k+1}^{x,k} - \textbf{I} \\
\cdots \\        
\end{bmatrix}^{-1}
\begin{bmatrix}
\textbf{R}_{y}^{x}\textbf{t}_{y,k}^{x,k-1} - \textbf{t}_{x,k}^{x,k-1} \\
\textbf{R}_{y}^{x}\textbf{t}_{y,k+1}^{x,k} - \textbf{t}_{x,k+1}^{x,k} \\
\cdots \\        
\end{bmatrix}\\
\end{split}
\label{equ.lls}
\end{equation}

The translation estimate is dependent highly on the accuracy of rotation matrix calculation and sensitive to noise in motion estimation. But in many instances, $\textbf{R}_{x,k}^{x,k-1} \approx \textbf{I}$ leads the left matrix approximate to $\textbf{0}$. Dividing by this matrix reduces the signal-to-noise ratio (SNR) and thus degrades the estimation. Consequently the translation estimates are less accurate than the rotation estimates \cite{taylor2016motion}. \\

In addition, due to uncertainty in motion estimation, we use random sample consensus (RANSAC) algorithm \cite{fischler1981random} to reject outliers. Please see line 9-13 or line 15-19 for detailed steps.\\

\subsubsection{Refinement}
In this step, we implement a registration algorithm (appearance-based approach) to improve the calibration results of the above motion-based approach further.  In this paper, we use the GICP \cite{segal2009generalized} as our registration algorithm. The key benefit of the last step is removing the initialization need for the registration method. Since the objective is non-convex, the algorithm will be stuck in a local minima without a good initial guess. 

\begin{algorithm}
	\caption{Proposed calibration method}
	\begin{algorithmic}[1]
		\REQUIRE Point clouds from $N$ lidars at timestamp $k$: $\mathcal{P}_{k}^{L_i}$.
		\ENSURE Extrinsic parameters from $L_1$ to $L_i$ : $\underset{1\leq i\leq N}{\bigcup}\{(\textbf{R}_{L_i}^{L_1})^{*}, (\textbf{t}_{L_i}^{L_1})^{*}\}$,
		\FOR {each timestamp $k$}
			\STATE $\textbf{R}_{L_i,k}^{L_i,k-1}$, $\textbf{t}_{L_i,k}^{L_i,k-1} \leftarrow $ \textit{motion-estimation}($\mathcal{P}_{k-1}^{L_i}$, $\mathcal{P}_{k}^{L_i}$); 
		\ENDFOR
		\FOR {each lidar $L_{i}$}
			\STATE $\mathcal{T}^{L_i}\leftarrow\underset{1\leq k\leq K}{\bigcup}\{\textbf{R}_{L_i,k}^{L_i,k-1},\textbf{t}_{L_i,k}^{L_i,k-1}\}$;
			\STATE $\mathcal{T}^{L_i}_\textbf{R}\leftarrow\underset{1\leq k\leq K}{\bigcup}\{\textbf{R}_{L_i,k}^{L_i,k-1}\}$;
			\FOR {each loop} 		
				\STATE $(\mathcal{T}^{L_i}_{\textbf{R}})^{'},(\mathcal{T}^{L_i}_{\textbf{R}})^{'}\leftarrow \textit{data-sample}\left(\mathcal{T}^{L_i}_{\textbf{R}}, \mathcal{T}^{L_i}_{\textbf{R}}\right)$;
				\STATE $\textbf{R}_{L_i}^{L_1} \leftarrow \textit{Kabsch}\left[(\mathcal{T}^{L_i}_{\textbf{R}})^{'},(\mathcal{T}^{L_i}_{\textbf{R}})^{'}\right]$;
				\STATE $n_{\text{inlier}} \leftarrow \textit{inlier-number}\left(\mathcal{T}^{L_i}_{\textbf{R}},\mathcal{T}^{L_i}_{\textbf{R}},\textbf{R}_{L_i}^{L_1}\right)$;
			\ENDFOR
			\STATE $\textbf{R}_{L_i}^{L_1} \leftarrow \textit{rotation-with-maximum-inlier}\left(\textbf{R}_{L_i}^{L_1},n_{\text{inlier}}\right)$;
			\FOR {each loop}		
				\STATE $(\mathcal{T}^{L_1})^{'},(\mathcal{T}^{L_i})^{'}\leftarrow \textit{data-sample}\left(\mathcal{T}^{L_1}, \mathcal{T}^{L_i}\right)$;
				\STATE $\textbf{t}_{L_i}^{L_1}\leftarrow \textit{linear-least-square}\left[(\mathcal{T}^{L_1})^{'},(\mathcal{T}^{L_i})^{'},\textbf{R}_{L_i}^{L_1}\right]$;
				\STATE $n_{\text{inlier}}\leftarrow \textit{inlier-number}\left(\mathcal{T}^{L_1},\mathcal{T}^{L_i},\textbf{t}_{L_i}^{L_1}\right)$;
			\ENDFOR		
			\STATE $\textbf{t}_{L_i}^{L_1}\leftarrow \textit{translation-with-maximum-inlier}\left(\textbf{t}_{L_i}^{L_1},n_{\text{inlier}}\right)$;				
			\STATE $(\textbf{R}_{L_i}^{L_1})^{*}, (\textbf{t}_{L_i}^{L_1})^{*} \leftarrow \textit{registration}\left(\mathcal{P}_{K}^{L_1}, \mathcal{P}_{K}^{L_i}, \textbf{R}_{L_i}^{L_1}, \textbf{t}_{L_i}^{L_1}\right)$;
		\ENDFOR
	\end{algorithmic}
	\label{alg.proposed_method}    
\end{algorithm}

\begin{comment}
	Denote the set of relative transformations of lidar $L_1$: 
	$\mathcal{T}^{L_i}$
	=
	$\underset{1\leq k\leq K}{\bigcup}\left\{\textbf{R}_{L_i,k}^{L_i,k-1},\textbf{t}_{L_i,k}^{L_i,k-1}\right\}$,
	$\mathcal{T}^{L_i}_{\textbf{R}}$=$\underset{1\leq k\leq K}{\bigcup}\left\{\textbf{R}_{L_i,k}^{L_i,k-1}\right\}$.
	\\
\end{comment}








==> criticism.tex <==
\section{Criticism of the Existing Work}
\label{criticism}

Determining which approaches are the best is not an easy job. To evaluate a calibration method, various factors should be considered: efficiency, generality, whether or not a calibrated marker is needed. The appearance-based make use of the surrounding information to find data association, but they are restricted to a particular type of sensor pair, like multi-lidar, or lidar-camera. Especially, most of appearance-based approaches can only work on sensors with overlapping fields of view.
On the contrary, motion-based approaches can generally calibrate the multimodal sensor. However, new issues appear because the accuracy of these approaches is highly dependent on the range of motion and the motion estimation of each sensor. Therefore, the system should undergo sufficient motion in structured environments to provide enough data to estimate the rotational and translational offset. 

\subsection{Appearance-Based Approaches}
The selection of the error metric for the ICP algorithm relies on the appearance of surroundings. The point-to-point \cite{besl1992method} is efficient in computation (having a closed-form solution), while the point-to-plane \cite{chen1992object} and the plane-to-plane \cite{segal2009generalized} are less sensitive to noise. The latter two metrics assume that most 3D data points are locally planar and can be described with plane normals. Thus they perform between in structured environments than the point-to-point metric. \\

The minimization of equ. (\ref{equ.icp_pointpoint}) and (\ref{equ.icp_pointplane}) can be optimized via a closed form solution, while in complicated cases like (\ref{equ.icp_planeplane}),  general non-linear least squares algorithms are more effective. In previous work, the Gauss-Newton approach \cite{spek2017joint} or the Levenberg-Marquardt algorithm \cite{fitzgibbon2003robust} have been utilized to minimize the error. However, these gradient-based approaches will converge to a  local minima if the objective is not globally convex. \\

To tackle this problem researchers have resorted other ways to improve the performance of ICP. One solution is to improve the quality of correspondences matching. In these work \cite{he2013pairwise, he2014calibration}, multi-type geometric features are extracted from the 3D maps to build a pair of correspondences.  Another solution is providing a proper initial guess on the extrinsic parameters. In \cite{pandey2017alignment, maroli2017automated}, the ground plane is utilized to align the point clouds in roll, pitch, and Z-axis offset. However, these solutions have strong assumptions on the structures of surroundings.







\subsection{Motion-Based Approaches}
Traditionally, many researchers have focused on finding efficient solutions to equation ($\ref{equ.hand_eye}$). In 1980's, the state-of-the-art solutions were separated into two opposite Directions: coupling and decoupling. The coupling approach operates on global nonlinear optimization, but it time-consuming in a large-scale case. On the contrary, the decoupling approach is more effective and gradually becomes a prominent solution in further years. Tsai et al. \cite{tsai1989new} derived a series of general geometric properties of the hand-eye calibration problem and proposed a  fast and accurate algorithm on the decoupling approach. Later, the computing procedure for rotation was improved in Kabsch's method \cite{kabsch1978discussion}. The Kabsch algorithm performs well even initial guess is not given. This algorithm can find an optimal solution with a minimum least squared error. \\

However, these methods are restricted in indoor environments where the sensors' motion is easily obtained. In more challenging cases, the uncertainty of motion should be considered. Therefore, Taylor et al. \cite{taylor2016motion} combined with appearance-based and motion-based approaches to present a complete calibration system for vehicles. This method is applicable in multimodal sensors and does not require any prior knowledge on the extrinsic parameters. The main contribution of it is building up a probabilistic framework to formulate the uncertainty of sensors' motion. By implementing an appearance-based approach (called Intensity-Motion Metric), the results of lidar-camera calibration are improved. As introduced in Section \ref{sec.overview}, this system consists of three steps: initialization, MLE and refinement. A non-linear least squares technique is utilized in the MLE step. Considering the objective is not convex, the initialization step is necessary to provide an initial guess. Motion-based approaches can be also employed on other platforms. In \cite{heng2013camodocal}, Heng et al. proposed a similar pipeline for multi-camera calibration. The novelty of this method is the usage of bundle adjustment for refinement. However, two limitations are posed in these work: the calibration problem of multi-lidar is still unsolved; they did not explain what a proper motion should look like.











==> overview.tex <==
\section{Overview of Existing Work}
\label{sec.overview}
 

The literature on multi-sensor calibration is divided into two separate areas: appearance-based and motion-based. To provide an in-depth review of the methods most relevant to our work, we limit the scope of the approaches that have been applied over multi-lidar, multi-camera and lidar-camera configurations.

\subsection{Appearance-Based Approaches}
\label{subsec.appearance_based}
These approaches are useful in several sensor configurations with exteroceptive sensors, like lidars and cameras, which operate on the appearance of the surroundings. The key to solving the calibration problem is to find data association from the measurements of different sensors.\\

In multi-lidar configurations, the process of finding data association is called registration (shown in Fig. \ref{fig.registration}), with a goal to find a transformation matrix to minimize the alignment error between two point clouds. Denoting $\textbf{p}^{L_i}_{k} \in \mathcal{P}^{L_i}$ as a 3D data point perceived by $L_i$, $\textbf{p}^{L_j}_{k} \in \mathcal{P}^{L_j}$ as the corresponding point perceived by $L_j$, registration is usually solved by implementing the following iterative closest point (ICP) algorithm \cite{besl1992method}:
\begin{equation}
	\begin{split}
		(\textbf{T}_{L_j}^{L_i})^{l+1} 
		= 
		\underset{\textbf{T}}{\text{minimize}}
		\sum_{k=1}^{K}
		E\left[(\textbf{T}_{L_j}^{L_i})^{l}\oplus(\textbf{p}^{L_i}_{k}), \textbf{p}^{L_j}_{k}\right], \ \ \ \ \ 
		\textbf{p}^{L_i}_{k} \in \mathcal{P}^{L_i}, \ \ \ \ \ 
		\textbf{p}^{L_j}_{k} \in \mathcal{P}^{L_j}.
		\\
	\end{split}
\end{equation}
Here $(\textbf{T}_{L_j}^{L_i})^{l+1}$ is the estimated transformation matrix from coordinate system $\{L_i\}$ to coordinate system $\{L_j\}$ at $l_{\text{th}}$ iteration, $\textbf{T}\oplus\textbf{p}$ denotes the Euclidean transformation of the point $\textbf{p}$. $E(\cdot,\cdot)$ is an error metric which has several variants: point-to-point \cite{besl1992method}, point-to-plane \cite{chen1992object} and plane-to-plane \cite{segal2009generalized}. Their definitions are given below:
\begin{align} 
	&\text{point to point}: E = \|\textbf{R}_{L_j}^{L_i}\textbf{p}^{L_i}_{k} + \textbf{t}_{L_j}^{L_i} - \textbf{p}^{L_j}_{k}\|^{2}, \label{equ.icp_pointpoint} \\
	&\text{point to plane}: E = (\textbf{R}_{L_j}^{L_i}\textbf{p}^{L_i}_{k} + \textbf{t}_{L_j}^{L_i} - \textbf{p}^{L_j}_{k})\cdot \textbf{n}_{k}^{L_j}, \label{equ.icp_pointplane} \\
	&\text{plane to plane}: E = \|\textbf{R}_{L_j}^{L_i}\textbf{p}^{L_i}_{k} + \textbf{t}_{L_j}^{L_i} - \textbf{p}^{L_j}_{k}\|_{\textbf{C}}, \ \ \ \ \ 
	\textbf{C} = \textbf{R}_{L_j}^{L_i}\text{cov}(\mathcal{P}^{L_i})(\textbf{R}_{L_j}^{L_i})^{-1}+
	\text{cov}(\mathcal{P}^{L_j}). \label{equ.icp_planeplane}
\end{align}

\bigskip
An example is \cite{he2013pairwise}, He et al. developed a method of calibrating a multiple 2D lidar sensing system based on ICP, which can be conducted in a general outdoor environment without any modification of the environment. This method extracts geometric features such as point, lines, planes, and quadrics from 3D maps instead of a single point cloud. However, it relies on a global navigation satellite system (GNSS) to build 3D maps, which will limit its further application. To cope with this problem, the authors proposed an extended version which uses 2D Simultaneous localization and mapping (SLAM) not GNSS for mapping\cite{he2014calibration}.\\
\begin{figure}[]
	\centering
	\begin{minipage}[t]{0.35\textwidth}
		\centering
		\includegraphics[height=0.6\textwidth]{image/introduction/registration-crop.pdf}
		\caption{An example of point cloud registration.}
		\label{fig.registration}				
	\end{minipage} \hspace{1cm}		
	\begin{minipage}[t]{0.35\textwidth}
		\centering
		\includegraphics[height=0.5\textwidth]{image/introduction/ground_alignment-crop.pdf}
		\caption{This figure shows the axis and angle pair that aligns the unit normal vectors corresponding to planes $\textbf{P}$ and $\textbf{Q}$. The angle from $\textbf{n}_{q}$ to $\textbf{n}_{p}$ is given by $\theta$. The rotation axis $\vec{k}$ is defined by the two normals $\textbf{n}_{q}$ and $\textbf{n}_{p}$.}
		\label{fig.ground_alignment}				
	\end{minipage}%
\end{figure}

Several registration approaches \cite{pandey2017alignment} assume that the point clouds captured by lidars should have a dominant ground plane perpendicular to the Z direction, which can also be used for calibration \cite{maroli2017automated}. By estimating the normals of the ground planes, the rotational offsets in X and Y axes can be found. Fig. \ref{fig.ground_alignment} shows the relationship between unit normals and rotation. Denoting $\textbf{n}_{1}$ and $\textbf{n}_2$ are unit normals of two planes, the angle $\theta$ and rotation axis $\textbf{k}$ are calculated:
\begin{equation}
	\begin{split}
		\textbf{k} = \textbf{n}_1 \times \textbf{n}_2, \ \ \ \ \ 
		\theta = \arccos(\textbf{n}_1 \cdot \textbf{n}_2).
	\end{split}
\end{equation}

By introducing Rodrigues rotation formula, the rotation matrix $\textbf{R}$ is calculated by its rotation axis $\textbf{k}$:
\begin{equation}
	\begin{split}
		\textbf{R} = \textbf{I} + \sin(\theta)\textbf{Skew}({\textbf{k}}) + \left[1-\cos(\theta)\right]\textbf{Skew}({\textbf{k}})^{2}.
	\end{split}
\end{equation}

The skew-symmetric matrix generated by a vector $\textbf{k}$ is 
\begin{equation}
	\begin{split}
		\textbf{Skew}({\textbf{k}}) = 
		\begin{bmatrix}
		0 & -k_z & k_y \\
		k_z & 0 & -k_x \\
		-k_y & k_x & 0 \\
		\end{bmatrix}.		
	\end{split}
\end{equation}		

Placing markers in the scene is a widely used technique in several calibration approaches \cite{geiger2012automatic, unnikrishnan2005fast, xie2018infrastructure} since markers can provide clear data association between sensors. Zhou et al. \cite{zhouautomatic} proposed an extrinsic calibration approach for a lidar-camera configuration. They extracted line and plane features from a chessboard to associate the measurements between sensors. \cite{xie2018infrastructure} presented a calibration environment consisting a large amount of Apriltags. Based on it, a unified calibration framework was realized for multi-lidar and multi-camera calibration.






\subsection{Motion-Based Approaches}
\label{subsec.motion_based}
Already introduced in Section \ref{sec.introduction}, motion-based approaches are grown from the hand-eye calibration problem.
Its basic form: $\textbf{AX=XB}$ has been well understood since relevant solutions were proposed \cite{horaud1995hand,tsai1989new,kabsch1978discussion}. In the late 1980s, an efficient solution was given in \cite{tsai1989new}, where the authors decoupled the computing procedure of rotational and translational components. By using a property of a rotation matrix is that its rotation axis is its eigenvector with eigenvalues equal to 1. Denoting rotation axes of $\textbf{R}_{x,k}^{x,k-1}$, $\textbf{R}_{y,k}^{y,k-1}$ and $\textbf{R}_{y}^{x}$ as $\textbf{r}_{x,k}^{x,k-1}$, $\textbf{r}_{y,k}^{y,k-1}$ and $\textbf{r}_{y}^{x}$ respectively, we start by equ. (\ref{equ.hand_eye_1}):
\begin{equation}
	\begin{split}
		\textbf{R}_{x,k}^{x,k-1}\textbf{R}_{y}^{x}\textbf{r}_{y,k}^{y,k-1} &=
		\textbf{R}_{y}^{x}\textbf{R}_{y,k}^{y,k-1}\textbf{r}_{y,k}^{y,k-1} \Rightarrow
		\textbf{R}_{x,k}^{x,k-1}\textbf{r}_{x,k}^{x,k-1} =
		\textbf{R}_{y}^{x}\textbf{r}_{y,k}^{y,k-1}
	\end{split}
\end{equation}
$\Rightarrow$
\begin{equation}
	\label{equ.rotation_axes}
	\begin{split}
		\textbf{r}_{x,k}^{x,k-1} = \textbf{R}_{y}^{x}\textbf{r}_{y,k}^{y,k-1}.
	\end{split}
\end{equation}
Therefore, we can set up a system of linear equations about rotation at each timestamp::
\begin{equation}
	\label{equ.ls_rotation}
	\begin{split}
		\textbf{Skew}(\textbf{r}_{x,k}^{x,k-1} + \textbf{r}_{y,k}^{y,k-1}) (\textbf{r}_{y}^{x})^{'}
		=
		\textbf{r}_{x,k}^{x,k-1} - \textbf{r}_{y,k}^{y,k-1}, \ \ \ \ \ 
		k\in\{1,2,\dots, K\}.
	\end{split}
\end{equation}
Where $\textbf{Skew}(\textbf{r}_{x,k}^{x,k-1} + \textbf{r}_{y,k}^{y,k-1})$ is a singular matrix \cite{tsai1989new}, $(\textbf{r}_{y}^{x})^{'}=
\frac{1}{\sqrt{4-|\textbf{r}_{y}^{x}|^{2}}}\textbf{r}_{y}^{x}$. The rotation angle is calculated:
\begin{align}
	\theta_{y}^{x} 
	&= 
	-2\text{ tan}^{-1}|(\textbf{r}_{y}^{x})^{'}|
\end{align}
Once the rotation matrix is found, we can also give a system of linear equations about translation at each timestamp:
\begin{align}
	\label{equ.ls_translation}
	(\textbf{R}_{x,k}^{x,k-1} - \textbf{I}) \textbf{t}_{y}^{x} 
	&= 
	\textbf{R}_{y}^{x}\textbf{t}_{y,k}^{y,k-1} - \textbf{t}_{x,k}^{x,k-1},\ \ \ \ \ 
	k\in\{1,2,\dots, K\}.
\end{align}
Given at least tow pairs of transformations at different timestamps, both equ. ($\ref{equ.ls_rotation}$) and ($\ref{equ.ls_translation}$) can be solved with linear least squares solutions.\\

Another technique to determine an optimal rotation matrix between two sets of vectors is called Kabsch algorithm \cite{kabsch1978discussion}.  This method operates on the covariance matrix to find the rotation between two sets of vectors. Denoting the vector sets  as $\textbf{P}$ and $\textbf{Q}$, cross-covariance matrix as $\textbf{H}$, $\textbf{R}$ is calculated:
\begin{equation}
	\label{equ.kabsch}
	\begin{split}
		\textbf{R} = (\textbf{H}^{T}\textbf{H})^{\frac{1}{2}}\textbf{H}^{-1},
		\ \text{with} \ 
		\textbf{H} = \textbf{P}^{T}\textbf{Q}.
	\end{split}
\end{equation}
Since $\textbf{H}$ is not always singular, singular value decomposition (SVD) is introduced:
\begin{equation}
	\label{equ.kabsch_svd}
	\begin{split}
		\textbf{H} = \textbf{U}\textbf{S}\textbf{V}^{T}, \ \ \ \ \ 	
		\textbf{R} = \textbf{V}
		\begin{bmatrix}
			1 & 0 & 0 \\
			0 & 1 & 0 \\
			0 & 0 & d \\
		\end{bmatrix}
		\textbf{U}^{T}
		\ \text{with} \ 
		d = \det(\textbf{V}\textbf{U}^{T}).\\
	\end{split}
\end{equation}

However, the above-described techniques have the disadvantages of requiring calibrated markers to be placed in the scene to estimate the sensor's motion. In many applications, the uncertainty of motions should be counted. Taylor et al. \cite{taylor2016motion} presented a calibration system for multimodal sensors within a robust probabilistic framework. After obtaining the motions of sensors, this method mainly divides the process of parameters estimates into three steps: initialization, maximum likelihood estimation (MLE) and appearance-based refinement. In the initialization step, the estimated values  $\textbf{R}_{y}^{x}$ and $\textbf{t}_{y}^{x}$ are accomplished by applying the Kabsch algorithm with additional non-equal weights assigned to the motions at each timestamp:
\begin{equation}
	\begin{split}
		W_k = \frac{1}{\sqrt{
				\left[
				\sum_{i=1}^{3}\text{cov}(\textbf{r}_{x,k}^{x,k-1})_{i,i}\right] 
				+
				\left[\sum_{i=1}^{3}\text{cov}(\textbf{r}_{y,k}^{y,k-1})_{i,i}\right]		
				}}.
	\end{split}
\end{equation}
where $\text{cov}(\textbf{r})\in \mathbb{R}^{3\times3}$ is the covariance matrix of $\textbf{r}$. 
Given the initial guess, the uncertainty of rotation estimates is formulated using Gaussian distribution:
\begin{equation}
	\begin{split}
		\textbf{r}_{y, k}^{y, k-1} -  \textbf{R}_{y}^{x}\textbf{r}_{x,k}^{x,k-1}
		\sim 
		\mathcal{N}(\boldsymbol{\textbf{0}}, \Sigma), \ \ \ \ \
		\Sigma 
		= 
		\text{cov}(\textbf{R}_{err})
		=
		\text{cov}(\textbf{R}_{y}^{x}) + \textbf{R}_{y}^{x}\text{cov}(\textbf{R}_{x,k}^{x,k-1}) (\textbf{R}_{y}^{x})^{T}.
	\end{split}
\end{equation}
Similarly, the uncertainty of translation estimates is expressed as follows:
\begin{equation}
	\begin{split}
		(\textbf{R}_{x,k}^{x,k-1} - \textbf{I}) \textbf{t}_{y}^{x} 
		-
		\textbf{R}_{y}^{x}\textbf{t}_{y,k}^{y,k-1} - \textbf{t}_{x,k}^{x,k-1}
		\sim 
		\mathcal{N}(\textbf{0}, \Sigma), \ \ \ \ \
		\Sigma 
		= 
		\text{cov}(\textbf{t}_{err}).
	\end{split}
\end{equation}

Denoting the likelihoods of sensors' motion as $\mathcal{L}_{\textbf{R}}(x,y,k)$ and $\mathcal{L}_{\textbf{t}}(x,y,k)$, the MLE step builds up an optimization problem by maximizing the log-likelihood sums over motion of $N$ sensors at all timestamps:
\begin{equation}
	\begin{split}
		\{\textbf{R}^{*}, \textbf{t}^{*}\} 
		= 
		\underset{\{\textbf{R}, \textbf{t}\}}{\text{argmin}}
		\left[
		\sum_{x=1}^{N}\sum_{y=1}^{N}\sum_{k=1}^{K}\log\mathcal{L}_{\textbf{R}}(x,y,z)
		+
		\sum_{x=1}^{N}\sum_{y=1}^{N}\sum_{k=1}^{K}\log\mathcal{L}_{\textbf{t}}(x,y,z)	
		\right].
	\end{split}
\end{equation}

Finally, the appearance-based step is combined since the accuracy of the motion-based approaches depends on the motion and sensors used. As discussed in Section \ref{subsec.appearance_based}, many appearance-based approaches have been proposed on different sensor configurations. In this paper, the authors used the intensity-motion metric to refine lidar-camera calibration. \\

Another motion-based approach for multi-sensor calibration is \cite{heng2013camodocal}, where four cameras without overlapping fields of view are calibrated. In this method, visual odometry of each camera is combined with a car's motion to give a coarse estimation of the extrinsic parameters. Bundle adjustment is then performed to refine the parameters. In contrast to \cite{taylor2016motion}, rotation was expressed in quaternions instead of matrices. \\


























==> preliminary.tex <==
 

==> preliminary_idea.tex <==
\section{Preliminary Ideas} 
The problem addressed in this paper is to estimate the extrinsic calibration parameters between 3D lidars \footnote{\url{https://velodynelidar.com/vlp-16.html}}  which are mounted on a vehicle. To make it simple, we make the following assumptions:
\begin{enumerate}
	\item The lidars data are synchronized;
	\item The motion of lidars are known, which can be represented by different types, such as a $4\times 4$ transformation matrix in Euclidean space;
	\item The lidars undergo a series of nondegenerate transformation;	
	\item The lidars are rigid mounting;
	\item The number of lidars $N=2$.
\end{enumerate}

\begin{comment}
\begin{figure}[]
	\centering
	\includegraphics[height=0.2\textwidth]{image/introduction/lidar-crop.pdf}%
	\caption{3D lidar}		
	\label{fig.lidar}
\end{figure}
\end{comment}	

Let us give some notations as follows:
\begin{equation}
	\begin{split}
		\textbf{T}_{y}^{x} \in \mathbb{R}^{4\times4} :& \text{ The transfomation from the frame of sensor }x\text{ to the frame of sensor }y \\
		\textbf{T}_{o,j}^{o,i} \in \mathbb{R}^{4\times4}:& \text{ The transfomation from the odometry frame } \text{ at timestep } i \text{ to the odometry}\\
		&\text{ frame at timestamp } j\\	
		L_1, L_2, \dots L_N :& \text{ The lidar. } \text{In this paper, the frame of } L_1 \text{ is considered as the odometry frame}
	\end{split}
\end{equation}

With assumptions and notations made, our calibration problem can be defined as a extended version of the standard hand-eye calibration problem: Given a sequence of lidar transformations $\textbf{T}_{L_i,k}^{L_i,k-1}, k \in \left\{0, 1,\dots, K\right\}$, compute the relative transformation from the frame of $L_1$ to the frame of other lidars $\textbf{T}_{L_i}^{L_1}$.

Fig.\ref{fig.hand_eye_calibration_vehicle} shows a depiction of how each sensors' motion and relative position are related on a vehicle. As the vehicle moves, $\textbf{T}_{L_i}^{L_1}$ can be recovered by using the transformations at each timestamp:
\begin{equation}
	\textbf{T}_{L_1,k}^{L_1,k-1}\textbf{T}_{L_i}^{L_1} = \textbf{T}_{L_i}^{L_1}\textbf{T}_{L_i,k}^{L_i,k-1}
\end{equation}

\begin{figure}[]
	\centering
	\includegraphics[height=0.3\textwidth]{image/introduction/hand_eye_calibration_vehicle-crop.pdf}
	\caption{The transformation of the lidars on a vehicle at timestamp $k$}		
	\label{fig.hand_eye_calibration_vehicle}
\end{figure}

The equ.(\ref{equ.hand_eye}) can be written into two equations by decomposing
$\textbf{T} = 
\begin{bmatrix}
	\textbf{R} & \textbf{t} \\
	\textbf{0} & 1 \\
\end{bmatrix}$,
\begin{align} 
	\textbf{R}_{L_1,k}^{L_1,k-1}\textbf{R}_{L_i}^{L_1} &=
	\textbf{R}_{L_i}^{L_1}\textbf{R}_{L_i,k}^{L_i,k-1} \label{equ.hand_eye_1} \\
	\textbf{R}_{L_i}^{L_1}\textbf{t}_{L_1,k}^{L_1,k-1} + \textbf{t}_{L_i}^{L_1} &= 
	\textbf{R}_{L_i,k}^{L_i,k-1}\textbf{t}_{L_i}^{L_1} + \textbf{t}_{L_i,k}^{L_i,k-1} \label{equ.hand_eye_2} 
\end{align}

where $\textbf{R} \in \mathbb{R}^{3\times3}$ are the rotation matrices and $\textbf{t} \in \mathbb{R}^{3}$ are the translation vectors. Specifically, $\textbf{R}$ are square and orthogonal with such special properties $\textbf{R}^{T}\textbf{R} = \textbf{I}$ and $\det\textbf{R}=\textbf{I}$.

By combining equ.(\ref{equ.hand_eye_1}) with (\ref{equ.hand_eye_2}), we can write down an optimization problem with an equality constraint on $\textbf{R}_{L_2}^{L_1}$:
\begin{equation}
	\label{equ.optimization}
	\begin{split}
		\underset{\textbf{R}_{L_2}^{L_1}, \textbf{t}_{L_2}^{L_1}}{\text{minimize }} 
		& 
		\sum_{k=2}^{K}
		\left(
		\textbf{R}_{L_1,k}^{L_1,k-1}\textbf{R}_{L_i}^{L_1} -		\textbf{R}_{L_i}^{L_1}\textbf{R}_{L_i,k}^{L_i,k-1}
		\right)\\
		+
		&
		\sum_{k=2}^{K}		
		\left[\left(\textbf{R}_{L_2,k}^{L_2,k-1}-\textbf{I}\right)\textbf{t}_{L_2}^{L_1} 
		+ \textbf{t}_{L_2,k}^{L_2,k-1}- \textbf{R}_{L_2}^{L_1}\textbf{t}_{L_1,k}^{L_1,k-1}\right]\\
		\text{subject to } &\left(\textbf{R}_{L_2}^{L_1}\right)^{T}\textbf{R}_{L_2}^{L_1} = \textbf{I} \\
		&
		\det\textbf{R}_{L_2}^{L_1} =\textbf{I}
	\end{split}	
\end{equation}

This optimization problem has been solved in previous works \cite{taylor2016motion}, \cite{heng2013camodocal}. Considering $\textbf{t}_{L_2}^{L_1}$ is unconstrained, $\textbf{R}_{L_2}^{L_1}$ can be firstly optimized by minimizing the first term of the objective. Based on these works, this paper will present the following contributions:
\begin{enumerate}
	\item I will take the advantages of Lie ground and algebra to solve the problem (6).
	\item I will do experiments on different sensor motions.
	\item I will compare the proposed method with previous works in time complexity with numerical results.
\end{enumerate}



==> result.tex <==
\section{Numerical Results} 
\label{sec.result}
In this section, we demonstrate the accuracy of proposed extrinsic calibration. All experiments are presented with simulated datasets \footnote{\url{https://www.osrfoundation.org/simulated-car-demo/}}.

\subsection{Experimental Setup}
The simulation software is built using ROS Kinetic \cite{quigley2009ros} and Gazebo 8 \cite{koenig2004design}, which contains a simulated vehicle and roads (Fig.\ref{fig.simulation}). This vehicle is equipped with different sensors including 2D and 3D lidars, ultrasonic sensors, cameras. We select this system as it can provide synchronized sensor data and motion's ground truth. In experiments, we focus on three lidars calibration, i.e., $N=3$. 
These lidars are mounted on the front, roof, and back position respectively (Fig.\ref{fig.simulated_vehicle}), which can provide a wide range of observations with a little blind zone. The data output frequency of three lidars is at 10 Hz. 

\begin{figure}[h!]
	\centering
	\begin{minipage}[t]{0.4\textwidth}
		\centering
		\includegraphics[height=0.5\textwidth]{image/introduction/simulation-crop.pdf}
		\caption{A screenshot of the simulation software.}
		\label{fig.simulation}                
	\end{minipage} \hspace{1cm}  
	\begin{minipage}[t]{0.4\textwidth}
		\centering
		\includegraphics[height=0.5\textwidth]{image/introduction/simulated_vehicle-crop.pdf}
		\caption{A figure shows the coordinate systems of three lidars.}
		\label{fig.simulated_vehicle}                
	\end{minipage} 
\end{figure}

\subsection{Extrinsic Calibration Results}
We evaluate the proposed method using different datasets. Datasets are collected by driving the vehicle along with 4 different trajectories which contain synchronized point clouds (perceived by three lidars) and ground truth (lidars' motion and extrinsic parameters). Fig. \ref{fig.trajectory} shows the movements of the vehicle in the world coordinate. Each trajectory lasts from x seconds. The extrinsic parameters from $L_1$ to other lidars we set are shown in Table \ref{tab.extrainsic_parameters}.  $100$ trials are conducted for each trajectory. The calibration results are shown in Fig. \ref{fig.result_box_plot}. Our algorithm can successfully calibrate the rotational and translational offset in the first three trajectories with low absolute error, but fail in the past trajectories. The failure reason is that the last trajectory does not contain enough turns. As Section \ref{subsubsec.initialization} states, the accuracy of rotation and translation estimates is sensitive to the degeneracy of motion.

\begin{figure}[h!]
	\centering
	\includegraphics[height=0.28\textwidth]{image/introduction/trajectory-crop.pdf}
	\caption{Trajectories 1-4 (left to right) of vehicle's movement in the world coordinate system. Each trajectory performs different numbers of tight turns over an uneven surface.}            
	\label{fig.trajectory}
\end{figure}

\begin{table}[]
	\centering
	\caption{The ground truth of extrinsic parameters from $L_1$ to other lidars.}
	\begin{tabular}{|r|r|r|}
		\hline
		Lidar  & $L_2$ & $L_3$\\ \hline
		x [m] & $2.2$ &  $-2$ \\ 
		y [m] & $0$ &  $-2$ \\
		z [m] & $-0.8$ &  $-1$ \\
		roll [rad] & $0$ &  $0$ \\
		pitch [rad] & $0$ &  $0$ \\
		yaw [rad] & $0$ &  $\pi$ \\ \hline
	\end{tabular}
	\label{tab.extrainsic_parameters}
\end{table}

\begin{figure}[]
	\centering
	\caption{Box plots of the error in rotation in rad and translation in meters for optimization with different motion. Each experiment is repeated 100 times.}        
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_2$ on trajectory $1$.]{        
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_1_boxplot_lidar_1_2-crop.pdf}}
	\end{minipage}
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_3$ on trajectory $1$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_1_boxplot_lidar_1_3-crop.pdf}}
	\end{minipage}     
	
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_2$ on trajectory $2$.]{            
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_2-crop.pdf}}
	\end{minipage} 
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_3$ on trajectory $2$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_3-crop.pdf}}
	\end{minipage}     
	
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_2$ on trajectory $3$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_2-crop.pdf}}
	\end{minipage} 
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_3$ on trajectory $3$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_3-crop.pdf}}
	\end{minipage}         
	
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_2$ on trajectory $4$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_2-crop.pdf}}
	\end{minipage} 
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\subfigure[Absolute calibration error from $L_1$ to $L_3$ on trajectory $3$.]{    
			\includegraphics[height=0.5\textwidth]{image/introduction/trajectory_2_boxplot_lidar_1_3-crop.pdf}}
	\end{minipage}             
	\label{fig.result_box_plot}
\end{figure}






